A Unifying Approach to Picture Automata

A directed acyclic graph (DAG) can represent a two-dimensional string or picture. We propose recognizing picture languages using DAG automata by encoding 2D inputs into DAGs. An encoding can be input-agnostic (based on input size only) or input-driven (depending on symbols). Three distinct input-agnostic encodings characterize classes of picture languages accepted by returning finite automata, boustrophedon automata, and online tessellation automata. Encoding a string as a simple directed path limits recognition to regular languages. However, input-driven encodings allow DAG automata to recognize some context-sensitive string languages and outperform online tessellation automata in two dimensions.

==> cycle/1dDAG.tex <==
\begin{center}
\footnotesize\sffamily
\tikz
[every node/.style = {draw, circle, minimum size=5mm, inner sep=0pt}]
\graph
{
S -> t -> r -> i -> n -> g -> D -> A -> G;
};
~~~
\tikz
[every node/.style = {draw, circle, minimum size=5mm, inner sep=0pt}]
\graph
{
P -> a -> t -> h -> D -> A -> G;
P -> [bend left] h;
D -> [bend left] G;
D -> [bend left] A;
};
\end{center}


==> cycle/stripe.tex <==
               $
               \anchor{b4}{\stateBW}
               \sharparrow
               \anchor{b1}{\stateWB}
	       \dots
           \qquad
               \anchor{b2}{\stateWB}
               \sharparrow
               \anchor{b3}{\stateBW}
	       \dots
               $
               \begin{tikzpicture}[remember picture,overlay]
                       \path (b1) edge[-latex,out=40,in=140] (b2)
                             (b3) edge[-latex,out=140,in=40] (b4);
               \end{tikzpicture}


==> def/edgesets.tex <==
\begin{definition}[Input blind edges]\label{def:blindedgesets}

\end{definition}


==> def/grammar-short.tex <==
% very cool but not used throughout the whole paper!
%%%%%%%%%%%%%%%5, or,
%%%%%%%%%%%%%%%5if at least one of its vertices is labeled by a nonterminal, thus
%%%%%%%%%%%%%%%5$|\{ v \mid \lab(v)  \in N \}| \geq 1$,
%%%%%%%%%%%%%%%5a \emph{proper} prefix-DAG.

\begin{definition}[\tbd{Regular DAG grammar, $\Lgram$, $\Lall$ \cite{daggrammar}}]\label{def:grammar}%
A \emph{regular DAG grammar}\footnote{Since regular DAG grammars
are equivalent to regular DAG automata,
an illustrative example of how the DAGs are handeled 
can be found in \cite{DBLP:conf/mol/Drewes17}.} is a triple $\gramdef$.
% consisting of
% the disjoint alphabets $N$ and $\Sigma$ of \emph{nonterminals} and 
% respectively, and a set $R$ of \emph{rules}.
Each \emph{rule} $r \in R$ is of the form $\alpha \sigmaarrow\beta$
where $\sigma \in \Sigma$ while
the \emph{head} $\alpha$ and the \emph{tail} $\beta$ are elements of $N^*$.
%
For the prefix DAGs $G$ and $G'$,
there exists a \emph{derivation step} $G\To_rG'$ using a rule $r$
if $G$ contains pairwise distinct vertices $v_1,\dots,v_k$
such that $\lab(v_1 \cdots v_k)=\alpha$.
In that case, $G'$ is obtained from $G$ by
% TODO: icalp2024reviewer1reject-2 l. 142, 143: what are "temporary vertices" formally?
% TODO yvo: intuition behind the temporary vertices is that it is a proper graph
\begin{itemize}
\item
  adding the vertex $v$ with its label $\lab(v)=\sigma$ % according to the rule $r$
\item
  by letting the edges, formerly pointing to  $v_1,\dots,v_k$,
  %$e_i = \IN(v_i)$ for $i \in [k]$
  now point to $v$, thus $\tar(\IN(v_i)) = v$,
\item
  deleting the temporary vertices $v_1,\dots,v_k$ and, in turn,
  %into a single vertex\footnote{Note that the case
  %$\alpha=\lambda$ and thus $k=0$ is included.
  %Thus, in this case, a new vertex is created by merging zero vertices.}
  %$v$ with $\lab(v)=\sigma$
\item
  adding the temporary vertices $w_1,\dots,w_j$ %to the graph $G$,
  labeled by their nonterminals $\lab(w_1\cdots w_j)=\beta$
\item
  by connecting them to the graph with the edges
  %$e_1,\dots,e_j$ as
  $(v, w_1),\dots(v,w_j)$.
  %where $\OUT(v)=e_1\cdots e_j$, $\IN(w_i)=e_i$ for all $i\in[j]$
\end{itemize}
%
A \emph{derivation} is a sequence of prefix DAGs%
\footnote{%
We extend the notation $\To_{r_1\cdots r_n}$ to $\To_E$,
where $E$ is an (extended) regular expression over rules:
if $L(E)$ denotes the language of sequences of rules denoted by $E$,
then ${\To_E}={\bigcup_{r_1\cdots r_n\in L(E)}\To_{r_1\cdots r_n}}$.}
$G_0\To_{r_1}G_1\To_{r_2}\cdots\To_{r_n}G_n$, 
also denoted by $G_0\To_{r_1\cdots r_n}G_n$.
The set of all such $G_n$ that are complete is denoted by $\Lall$.
The \emph{DAG language generated by $\gram$} is 
$\Lgram = \{G\in\D_\Sigma\mid\emptygraph\To^*_R G\}$,
the set of connected and complete DAGs that the grammar can derive,
where $\To^*_R$ denotes the reflexive and transitive closure
of ${\To_R}=\bigcup_{r\in R}{\To_r}$.
As usual, a rule is said to be \emph{useless}
if none of the derivations of DAGs in $L(\gram)$ employs this rule
and \emph{useful} if it does.
%
% icalp2024reviewer2: p.5 l.150: not sure what is a "distinct combination"
%%%The DAG grammar $\gram$ is \emph{deterministic} if,
%%%for every distinct combination $\alpha\sigmaArrow{}$
%%%with $\alpha\in N^*$ and $\sigma\in\Sigma$,
The DAG grammar $\gram$ is \emph{deterministic} if,
for every pair $\alpha\sigmaArrow{}$ in $N^*\!\times\Sigma$,
there exists at most one $\beta\in N^*$
such that $(\alpha \sigmaarrow\beta)\in R$. 
The DAG language generated by a deterministic DAG grammar, 
as well as a DAG automaton recognizing it,
is called \emph{top-down deterministic}.
By reversing the orientation of the edges,
%thus $\tar(v) = \src(v)$ and vice versa for all DAGs in language $L$,
we obtain its \emph{dual language}.
A language $L(\gram)$ of a deterministic DAG grammar
is called \emph{bottom-up deterministic} if its dual language is generated by $\gram$.
% TODO: bottom-up not defined, I think
% TODO. RDLdet is my invention? is top-down meant? 

The class $\RDL$ of \emph{regular DAG languages}
consists of all DAG languages generated by a regular DAG grammar (equivalently recognized by a regular DAG automaton).
The class $\RDLdet$ of \emph{regular deterministic DAG languages}
consists of all DAG languages and dual languages 
generated by regular deterministic DAG grammars (equivalently recognized by a regular deterministic DAG automaton). 

\end{definition}


==> def/rfa_sqeezed-boundary.tex <==
Both automata models defined below, $\RFA$ and $\BFA$,
were introduced by Fernau, Paramasivan, Schmid and Thomas~%
\cite{DBLP:journals/jcss/FernauPST18}.
Both $\RFA$ and $\BFA$ work as a finite state machine
(as a $\DFA$ in the deterministic and an $\NFA$ in the nondeterministic case)
equipped with a scanning strategy
%; c.f. scanning strategy for two-dimensional restarting tiling automata~%
\cite{DBLP:journals/ijfcs/PrusaM13}
which enables the automaton models to operate on two-dimensional input.
%which can be viewed as a total order $\prec$
%an the elements of the two-dimensional input string.
The scanning strategy serializes a boundary picture $\hat P$ into
a string $\hat p$ over $\Sigmasharp$.
Afterward, the picture $P$ is accepted
if the corresponding $\FSA$ accepts this serialized picture $\hat p$.
Both models scan their input picture horizontally row by row,
according to their respective scanning strategy.
However, they differ in their scanning directions:
An $\RFA$ proceeds uniformly from left to right,
this corresponds to the reading of Western texts
where the eye has to `jump'
from the end of a line the beginning of the next one.
A $\BFA$, on the other hand, proceeds like an ox plowing a field,
alternating its direction.

\begin{definition}[$\RFA$, $\BFA$]\label{def:rfabfa}
Both a (deterministic) \emph{returning finite automaton}      ($\RFA$)
and a  (deterministic) \emph{boustrophedon  finite automaton} ($\BFA$)
are given by a 6-tuple
$ A = ( Q , \Sigma, \delta , q_0, F , \# )$,
where
%%%% $Q$ is the finite set of states,
%%%%  $\Sigma$ is the input alphabet,
$\delta \subseteq Q \times  (\Sigma \cup \{\#\}) \times  Q$
is the transition relation (transition function
$\delta : Q \times  (\Sigma \cup \{\#\}) \to Q$).

Both automata models are equipped with a \emph{scanning strategy},
which defines a total order $\prec$ on the positions of a two-dimensional string.
Formally, for a boundary picture $\hat P$, a position $\hat P(i_2,j_2)$ follows immediately after the position $\hat P(i_1,j_1)$ when
% holds
%$S(i_1,j_1) \prec S(i_2,j_2)$ if and only if, in case of an
%\begin{itemize}
% the condition $(i_1+j_1 < i_2+j_2)$ is wrong
%\item $\RFA:$
%  $(i_1+j_1 < i_2+j_2) \lor (i_1 = i_2 \land i_1 < i_2)$
%  and in case of a
%%$(i < k) \lor (i = k \land j < l)$
%\item $\BFA:$
%$
%  (i_1+j_1 < i_2+j_2) \lor
%\bigl((i_1+j_1 \mod 2 = 0 \land j_1 < j_2) \lor
%     (i_1+j_2 \mod 2 = 1 \land j_1 > j_2)\bigr)
%$.
%\end{itemize}
\begin{itemize}
\item for an $\RFA$:
  $(i_2=i_1 \land j_2=j_1+1)$ or $(i_2=i_1+1 \land j_1=m+1 \land j_2=0)$
\item \begin{tabbing}
for a $\BFA$: \=
  $\left[i_2=i_1 \mbox{ and } (i_1 \mod 2 = 0 \land j_2<j_1) \lor (i_1 \mod 2 = 1 \land j_2>j_1)\right]$ or \\
  \> $\left[i_2=i_1+1 \text{ and } (i_1 \mod 2 = 0 \land j_2=j_1=0) \lor (i_1 \mod 2 = 1 \land j_2=j_1=m+1)\right]$.
\end{tabbing}
\end{itemize}
With
$M = ( Q , \Sigmasharp, \delta , q_0, F )$ being an $\NFA$ ($\DFA$),
the language $L$ accepted by $A$ is given as
\begin{displaymath}
\begin{array}{rcl}
L(A) = \{ P \in \Sigma^{m,n}
& \mid &
\text{for all }
m,n \in \mathbb{N}_0,
s_1 s_2
\cdots
s_{(m+2)(n+2)}
\in L(M) \text{ where the }
%i \in [m+1]_0 \text{ and } j \in [n+1]_0
\\
& & \mbox{symbols }
 s_1, \ldots, s_{(m+2)(n+2)} \mbox{ are from the positions according }\\
& & \mbox{to the total position ordering } \prec \ \}\\
\end{array}
\end{displaymath}
\end{definition}

We present an alternative but equivalent definition
of \cite{DBLP:journals/jcss/FernauPST18},
which serves as a characterization emphasizing both
the treatment of the boundary symbols as well as the scanning strategy.
It is easy to see that our modified definition does not change the expressive power of the automata models:
every state computed within the top or bottom boundary
could be computed within the first, resp. last row of the picture as well
and two consecutive boundary symbols $\#\#$ do not equip
an automaton with expressiveness since it can do the same in one step
while reading the squeezed single $\#$, see below.

Here, we defined scanning strategies on a boundary picture
with all four sides explicitly represented.
The original definition \cite{DBLP:journals/jcss/FernauPST18}, in contrast,
delimits pictures only on the left and right and even then,
it does not reference all those boundary symbols.
% In \cite{DBLP:journals/jcss/FernauPST18}, both the returning automaton and boustrophedon automaton start from the top left corner of the input picture and ends after scanning the whole last row of the picture.  In our modified definition the boustrophedon automaton starts at the top-right corner of the boundary picture.
Using boundary pictures uniformly across all automaton models
supports a coherent perspective
and facilitates their systematic comparison in Sect.~\ref{sec:comp}.
By limiting the boundary symbols to acting as a `fence' in the serialized
string, we mimic the behavior of the original definition easily:
\begin{displaymath}
\begin{array}{rcl}
L(A) = \{ P \in \Sigma^{m,n}
& \mid &
\text{for all }
m,n \in \mathbb{N}_0,
s_1 s_2
\cdots
s_{m\cdot(n+1)-1}
\in L(M) \text{ where the symbols }
%i \in [m+1]_0 \text{ and } j \in [n+1]_0
\\
& & 
 s_1, \ldots, s_{m\cdot(n+1)-1} \mbox{ are from the positions according to the position}\\
& & \mbox{ordering } \prec \mbox{ starting with position } \hat P(1,1) 
\mbox{ ending with position } \hat P(m,n)
\mbox{ }\\
& & \mbox{and with each block of boundary symbols \# squeezed to a single \# } \}\\
\end{array}
\end{displaymath}
Our modified definition allows us consider a canonical representation of a boundary picture $\hat P$ as a directed acyclic graph with nodes corresponding to positions of the boundary picture in Sect.~\ref{subsubsec:rfabfa}.

By making the scanning strategy explicit, our characterization
reveals its effect on the family of languages recognized by the models.
As a result of the explicit scanning strategy,
Sect.~\ref{subsubsec:dia} demonstrates that parameterizing it
enables the recognition of a wider range of picture languages.


==> tikz.tex <==
\usetikzlibrary{arrows.meta,automata,positioning}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{petri}
\usetikzlibrary{shapes}
\usetikzlibrary{calc}
\usetikzlibrary{shadows}

% petri nets
\tikzstyle{place}=[circle,draw,minimum size=2mm]
\tikzstyle{transition}=[rectangle,draw,fill=black,minimum width=6mm,inner ysep=1pt]
\tikzset{
	every token/.style={minimum size=1pt},
	token distance=3pt
	anchor=base,
}
\tikzset{
    vertex/.style={
      %state,
      draw, 
      circle,
      fill,
      % circular drop shadow,
      inner sep=0pt,
      outer sep=0pt,
      minimum size=1ex,
      text=white,
      color=blue,
    }
}

